Demonstration of a Multiresolution Schema Mapping System

Enterprise databases usually contain large and complex schemas. Authoring complete schema mapping queries in this case requires deep knowledge about the source and target schemas and is thereby very challenging to programmers. Sample-driven schema mapping allows the user to describe the schema mapping using data records. However, real data records are still harder to specify than other useful insights about the desired schema mapping the user might have. In this project, we develop a schema mapping system, PRISM, that enables multiresolution schema mapping. The end user is not limited to providing high-resolution constraints like exact data records but may also provide constraints of various resolutions, like incomplete data records, value ranges, and data types. This new interaction paradigm gives the user more flexibility in describing the desired schema mapping. This demonstration showcases how to use PRISM for schema mapping in a real database.

==> related.tex <==
\section{Related Work}\label{sec:related}
\jin{this part is not done, depending on the actual need, we will add or delete in the end}

\minisection{PBE program synthesis} Inductive Program Synthesis is frequently applied in domains~\cite{jin2017foofah,gulwani2011automating, jin2017foofahdemo,barowy2015flashrelate,qian2012sample,shen2014discovering,Wang2017,mottin2014exemplar,bonifati2017interactive} where the user is required to have high domain expertise. 

\minisection{Schema mapping systems} Previous research on schema mapping~\cite{qian2012sample,shen2014discovering,Wang2017,mottin2014exemplar,bonifati2017interactive} have proposed sample-driven techniques for schema mapping. These systems usually ask the user for complete data records in the desired schema, which can still be hard to specify if the user is not familiar with the database content. 
